Understanding Counterexamples for Relational Properties with DIbugger

Software verification is a tedious process that involves the analysis of multiple failed verification attempts, and adjustments of the program or specification. This is especially the case for complex requirements, e.g., regarding security or fairness, when one needs to compare multiple related runs of the same software. Verification tools often provide counterexamples consisting of program inputs when a proof attempt fails, however it is often not clear why the reported counterexample leads to a violation of the checked property. In this paper, we enhance this aspect of the software verification process by providing DIbugger, a tool for analyzing counterexamples of relational properties, allowing the user to debug multiple related programs simultaneously.

==> eptcsdata.tex <==
\providecommand{\firstpage}{6}
\providecommand{\publicationstatus}{E. De Angelis, G. Fedyukovich, N. Tzevelekos and M. Ulbrich (Eds.):\\
Sixth Workshop on Horn Clauses for Verification and Synthesis and\\ 
Third Workshop on Program Equivalence and Relational Reasoning.\\
EPTCS 296, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.296.4}{10.4204/EPTCS.296.4}}
\pdfoutput=1

